Measurements of CKM angles beta/phi_1 and alpha/phi_2 at the BABAR and Belle experiments

We report measurements of the CKM angles beta/phi_1 and alpha/phi_2 done by the BABAR and Belle experiments. Both experiments have collected large data samples, corresponding to a total of more than 1 billion of BBbar pairs, at the e^+e^- asymmetric-energy colliders PEP-II (SLAC) and KEK-B (KEK), respectively.

==> biblio.tex <==

\bigskip % extra skip inserted
% Create the reference section using BibTeX:
%\bibliography{basename of .bib file}
\begin{thebibliography}{9}   % Use for  1-9  references
%\begin{thebibliography}{99} % Use for 10-99 references

%1
\bibitem{SM} S.~Weinberg, \jprl{19}, 1264 (1967); 
  A.~Salam, ``Elementary Particle Physics'', edited by N.~Svartholm 
  (Almquist and Wiksells, Stockhol 1968), p. 367; 
  S.~Weinberg, \jprl{37}, 657 (1976). 

%2
\bibitem{CKM} N.~Cabibbo, \jprl{10}, 531 (1963); 
  M.~Kobayashi, M.~Maskawa, \progtp{49}, 652 (1973).

%3
\bibitem{PDG08} C.Amsler \etal\ \plb{667}, 1 (2008).

%4
\bibitem{pep2}
PEP-II Conceptual Design Report, SLAC-PUB-0418 (1993).

%5
\bibitem{kekb}
S.~Kurokawa and E.~Kikutani, \nima{499}, 1 (2003).

%6
\bibitem{babardetector}
\babar\ Collaboration, B.~Aubert \etal, \nima{479}, 1 (2002).

%7
\bibitem{belledetector}
Belle Collaboration, A.~Abashian \etal, \nima{479}, 117 (2002).

%8
\bibitem{sin2betaD}
  \babar\ Collaboration, B. Aubert \etal, \jprl{89}, 201802 (2002);
  Belle Collaboration, K. Abe \etal, \jprd{66}, 071102 (2002).

%9
\bibitem{Penguin}
Y.~Grossman and M.~P.~Worah, \plb{395}, 241 (1997);
D.~Atwood and A.~Soni, \plb{405}, 150 (1997);
M.~Ciuchini \etal, \jprl{79}, 978 (1997).

%10
\bibitem{london} 
D.~London and A.~Soni, \plb{407}, 61 (1997).

%11
\bibitem{Gross} 
Y. Grossman \etal, \jprd{68}, 015004 (2003).

%12
\bibitem{Gronau}
  C.-W.~Chiang \etal, \jprd{68}, 074012 (2003); 
  M.~Gronau \etal, \plb{596}, 107 (2004).

%13
\bibitem{BN} 
  M. Beneke and M. Neubert, \npb{675}, 333 (2003).

%14
\bibitem{BN2} 
  M.~Beneke, \plb{620}, 143 (2005);
  G.~Buchalla \etal, JHEP~{\bf 0509}, 074 (2005).

%15
\bibitem{Cheng}
  H.~Y.~Cheng \etal, \jprd{72}, 014006 (2005), \jprd{71}, 014030 (2005);
  S. Fajfer \etal, \jprd{72}, 114001 (2005).

%16
\bibitem{Zupan}
A.~R.~Williamson and J.~Zupan, \jprd{74}, 014003 (2006).

%17
\bibitem{golden}
M.~Ciuchini \etal, \jprl{95}, 221804 (2005).

%18
\bibitem{ccsBabar}
\babar\ Collaboration, B.~Aubert \etal, \jprl{99}, 171803 (2007).

%19
\bibitem{ccsBelle}
Belle Collaboration, K.-F.~Chen \etal, \jprl{98}, 031802 (2007).

%20
\bibitem{psiksBelle}
Belle Collaboration, H.~Sahoo \etal, \jprd{77}, 091103 (2008).

%21
\bibitem{HFAG}
Heavy Flavor Averaging Group,
\url{http://www.slac.stanford.edu/xorg/hfag/triangle/}, Winter 2008 update.

%22
\bibitem{dsdskBabar}
\babar\ Collaboration, B.~Aubert \etal, \jprd{74}, 091101 (2006).

%23
\bibitem{dsdskBelle}
Belle Collaboration, J.~Dalseno \etal, \jprd{76}, 072004 (2007).

%24
\bibitem{Jpsipi0Babar}
\babar\ Collaboration, B.~Aubert \etal, \jprl{101}, 021801 (2008).

%25
\bibitem{Jpsipi0Belle}
Belle Collaboration, S.~E.~Leo \etal, \jprd{77}, 071101 (2008).

%26
\bibitem{dsdsBabar}
\babar\ Collaboration, B.~Aubert \etal, \jprd{76}, 111102 (2007).

%27
\bibitem{ddBabar}
\babar\ Collaboration, B.~Aubert \etal, \jprl{99}, 071801 (2007).

%28
\bibitem{ddBelle}
Belle Collaboration, T.~Aushev \etal, \jprl{93}, 201802 (2004);
Belle Collaboration, S.~Fratina \etal, \jprl{98}, 221802 (2007);

%29
\bibitem{dcph0}
\babar\ Collaboration, B.~Aubert \etal, \jprl{99}, 081801 (2007).

%30
\bibitem{dalitzdhBabar}
\babar\ Collaboration, B.~Aubert \etal, \jprl{99}, 231802 (2007).

%31
\bibitem{dalitzdhBelle}
Belle Collaboration, P.~Krokovny \etal, \jprl{97}, 081801 (2006).

%32
\bibitem{GL} 
M.~Gronau and D.~London, \jprl{65}, 3381 (1990);
H.~J.~Lipkin \etal, \jprd{44}, 1454 (1991);
M.~Gronau, \plb{265}, 389 (1991).

%33
\bibitem{GrossAlpha}
Y.~Grossman and H.~R.~Quinn, \jprd{58} 017504 (1998);
J.~Charles, \jprd{59}, 054007 (1999);
M.~Gronau \etal, \plb{514}, 315 (2001).

%34
\bibitem{GZ} 
M.~Gronau and J.Zupan, \jprd{70}, 074031 (2004).

%35
\bibitem{PiPiBabar}
\babar\ Collaboration, B.~Aubert \etal, \jprl{99}, 021603 (2007);
\babar\ Collaboration, B.~Aubert \etal, \jprd{76}, 091102 (2007).

%36
\bibitem{PiPiBelle}
Belle Collaboration, H.~Ishino \etal, \jprl{98}, 211801 (2007).

%37
\bibitem{babar_rho0rho0}
\babar\ Collaboration, B.~Aubert \etal, \jprl{98}, 111801 (2007).

%38
\bibitem{RhoRhoBabar}
\babar\ Collaboration, B.~Aubert \etal, \jprd{76}, 052007 (2007).

%39
\bibitem{RhoRhoBelle}
Belle Collaboration, A.~Somov \etal, \jprd{76}, 011104 (2007).

\bibitem{BabarRho0Rho0}
\babar\ Collaboration, B.~Aubert \etal, arXiv:0708.1630.

\bibitem{BelleRho0Rho0}
Belle Collaboration, C.-C. Chiang \etal, arXiv:0808.2576.

%40
\bibitem{snyder_quinn}
A.~E.~Snyder and H.~R.~Quinn, \jprd{48}, 2139 (1993). 

%41
\bibitem{rhopiBabar}
\babar\ Collaboration, B.~Aubert \etal, \jprd{76}, 012004 (2007).

%42
\bibitem{rhopiBelle}
Belle Collaboration, A.~Kusaka \etal, \jprl{98}, 221602 (2007).
Belle Collaboration, A.~Kusaka \etal, \jprd{77}, 072001 (2008).

%43
\bibitem{a1pi}
M.~Gronau and J.~Zupan, \jprd{73}, 057502 (2006).

%44
\bibitem{a1pibabar}
\babar\ Collaboration, B.~Aubert \etal, \jprl{98}, 181803 (2007).

%45
\bibitem{CKMfit}
CKMfitter Group, J.~Charles \etal, Eur.\ Phys.\ J.\ C {\bf 41}, 1 (2005).

\end{thebibliography}


\end{document}
%
% ****** End of file template.aps ******


==> definitions.tex <==

\RequirePackage{xspace}

\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

\def\CP                {\ensuremath{C\!P}\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\btos    {\ensuremath{b \to s}\xspace}
\def\btod    {\ensuremath{b \to d}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\btosss    {\ensuremath{b \to \ssbar s}\xspace}

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace}
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\rhoz   {\ensuremath{\rho^0}\xspace}

\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace}
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}

\def\epem       {\ensuremath{e^+e^-}\xspace}

\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\FourS {\Y4S}

\def\pep2{PEP-II}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}
\providecommand{\dt}{\deltat}

\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\providecommand{\pvec}{{\bf p}}
\providecommand{\half}{\mbox{${1\over2}$}}

\newcommand{\etal}{{\em et al.}}

\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\ttag}{\ensuremath{t_{\rm tag}}}
\newcommand{\tcp}{\mbox{$t_{\CP}$}}
\newcommand{\thetaT}{\ensuremath{\theta_{\rm T}}}
\newcommand{\xf}{\mbox{${\cal F}$}}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}

\newcommand{\phikz}{\ensuremath{\phi \kern -0.16em \Kz}\xspace}
\newcommand{\fzkz}{\ensuremath{f_0(980) \kern -0.16em \Kz}\xspace}
\newcommand{\kpkmkz}{\ensuremath{\KpKm \kern -0.16em \Kz}\xspace}
\newcommand{\etaprkz}{\ensuremath{\etapr \kern -0.16em \Kz}\xspace}
\newcommand{\pizkzs}{\ensuremath{\piz \kern -0.16em \KS}\xspace}
\newcommand{\kzskzskzs}{\ensuremath{\KS\KS\KS}\xspace}
\newcommand{\kzskzs}{\ensuremath{\KS\KS}\xspace}
\newcommand{\rhozkzs}{\ensuremath{\rhoz \kern -0.16em \KS}\xspace}
\newcommand{\omegakzs}{\ensuremath{\omega \kern -0.16em \KS}\xspace}

\newcommand{\btokzskzs}{\ensuremath{\Bz \to \KS\KS}\xspace}

\newcommand{\msp}{\ensuremath{\phantom{-}}}
\newcommand{\PM}{\ensuremath{\kern -0.21em\pm\kern -0.21em}\xspace}

% A useful Journal macro
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}

\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}

\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\bf #1}}}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
\newcommand{\nima}      [1]  {\nimBaseA~A~{\bf #1}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf
      #1}}}


\def\Journal#1#2#3#4{{\it #1} {\bf #2}, #3 (#4)}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

